HATS-13b and HATS-14b: two transiting hot Jupiters from the HATSouth survey

We report the discovery of HATS-13b and HATS-14b, two hot-Jupiter transiting planets discovered by the HATSouth survey. The host stars are quite similar to each other (HATS-13: V = 13.9 mag, M* = 0.96 Msun, R* = 0.89 Rsun, Teff = 5500 K, [Fe/H] = 0.05; HATS-14: V = 13.8 mag, M* = 0.97 Msun, R* = 0.93 Rsun, Teff = 5350 K, [Fe/H] = 0.33) and both the planets orbit around them with a period of roughly 3 days and a separation of roughly 0.04 au. However, even though they are irradiated in a similar way, the physical characteristics of the two planets are very different. HATS-13b, with a mass of Mp = 0.543 MJ and a radius of Rp = 1.212 RJ, appears as an inflated planet, while HATS-14b, having a mass of Mp = 1.071 MJ and a radius of Rp = 1.039 RJ, is only slightly larger in radius than Jupiter.

==> HATS582-006_rvtable.tex <==
$ 77.90592 $ & $   -89.89 $ & $    27.00 $ & $  -23.0 $ & $   13.0 $ & $   0.417 $ & FEROS \\
$ 78.86766 $ & $   168.11 $ & $    24.00 $ & $   15.0 $ & $   12.0 $ & $   0.764 $ & FEROS \\
$ 114.77348 $ & $   171.11 $ & $    44.00 $ & $    5.0 $ & $   19.0 $ & $   0.742 $ & FEROS \\
$ 114.85948 $ & $   151.11 $ & $    27.00 $ & $    5.0 $ & $   13.0 $ & $   0.773 $ & FEROS \\
$ 116.65611 $ & $   -69.89 $ & $    26.00 $ & $   36.0 $ & $   13.0 $ & $   0.422 $ & FEROS \\
$ 117.60502 $ & $   140.11 $ & $    37.00 $ & $   41.0 $ & $   17.0 $ & $   0.765 $ & FEROS \\
$ 121.81588 $ & $  -137.89 $ & $    37.00 $ & $  -13.0 $ & $   17.0 $ & $   0.287 $ & FEROS \\
$ 125.91876 $ & $   142.11 $ & $    33.00 $ & $   14.0 $ & $   15.0 $ & $   0.770 $ & FEROS \\
$ 145.75487 $ & $    47.11 $ & $    37.00 $ & $  -10.0 $ & $   17.0 $ & $   0.940 $ & FEROS \\
$ 160.71709 $ & $  -147.10 $ & $    39.00 $ & $   -6.0 $ & $   29.0 $ & $   0.347 $ & Coralie \\
$ 161.81222 $ & $    95.90 $ & $    96.00 $ & $  -19.0 $ & $   37.0 $ & $   0.743 $ & Coralie \\
$ 164.54335 $ & $   190.90 $ & $    43.00 $ & $  140.0 $ & $   29.0 $ & $   0.730 $ & Coralie \\
$ 424.76755 $ & $   162.11 $ & $    33.00 $ & $   12.0 $ & $   15.0 $ & $   0.784 $ & FEROS \\
$ 492.58995 $ & $  -151.89 $ & $    37.00 $ & $   46.0 $ & $   17.0 $ & $   0.297 $ & FEROS \\
$ 618.55621 $ & $   127.90 $ & $    44.00 $ & $  -53.0 $ & $   32.0 $ & $   0.826 $ & Coralie \\
$ 619.56771 $ & $  -128.10 $ & $    68.00 $ & \nodata      & \nodata      & $   0.191 $ & Coralie \\
$ 620.56070 $ & $    81.90 $ & $    70.00 $ & $   68.0 $ & $   37.0 $ & $   0.550 $ & Coralie \\


==> HATS582-012_rvtable.tex <==
$ 53.29791 $ & $    84.91 $ & $    91.40 $ & \nodata      & \nodata      & $   0.711 $ & CYCLOPS \\
$ 56.26837 $ & $   -27.19 $ & $    23.00 $ & \nodata      & \nodata      & $   0.687 $ & CYCLOPS \\
$ 57.29641 $ & $  -204.59 $ & $    21.20 $ & \nodata      & \nodata      & $   0.025 $ & CYCLOPS \\
$ 59.28565 $ & $   362.01 $ & $    48.90 $ & \nodata      & \nodata      & $   0.678 $ & CYCLOPS \\
$ 77.83581 $ & $   116.30 $ & $    25.00 $ & $   -4.0 $ & $   13.0 $ & $   0.772 $ & FEROS \\
$ 78.82092 $ & $   -52.70 $ & $    28.00 $ & $   11.0 $ & $   13.0 $ & $   0.096 $ & FEROS \\
$ 79.84891 $ & $   -43.70 $ & $    24.00 $ & $   16.0 $ & $   12.0 $ & $   0.434 $ & FEROS \\
$ 80.78831 $ & $   225.02 $ & $    35.00 $ & $  -62.0 $ & $   26.0 $ & $   0.742 $ & Coralie \\
$ 81.83369 $ & $   -75.98 $ & $    38.00 $ & $   60.0 $ & $   26.0 $ & $   0.086 $ & Coralie \\
$ 81.92743 $ & $   -71.70 $ & $    26.00 $ & $   -2.0 $ & $   13.0 $ & $   0.117 $ & FEROS \\
$ 82.93245 $ & \nodata      & \nodata      & $   93.0 $ & $   32.0 $ & $   0.447 $ & Coralie \\
$ 83.89769 $ & $    51.30 $ & $    25.00 $ & $    2.0 $ & $   13.0 $ & $   0.764 $ & FEROS \\
$ 84.78165 $ & $  -101.98 $ & $    43.00 $ & $ -170.0 $ & $   29.0 $ & $   0.054 $ & Coralie \\
$ 85.85427 $ & $  -179.70 $ & $    28.00 $ & $  -28.0 $ & $   14.0 $ & $   0.407 $ & FEROS \\
$ 85.93485 $ & $  -228.98 $ & $    42.00 $ & $  -76.0 $ & $   29.0 $ & $   0.433 $ & Coralie \\
$ 86.93769 $ & $   -36.70 $ & $    37.00 $ & $    1.0 $ & $   17.0 $ & $   0.762 $ & FEROS \\
$ 88.85705 $ & $  -251.70 $ & $    32.00 $ & $  -47.0 $ & $   15.0 $ & $   0.393 $ & FEROS \\
$ 114.66035 $ & $   131.30 $ & $    30.00 $ & $ -620.0 $ & $   14.0 $ & $   0.870 $ & FEROS \\
$ 115.81404 $ & $   -50.70 $ & $    30.00 $ & $ -116.0 $ & $   14.0 $ & $   0.249 $ & FEROS \\
$ 116.76798 $ & $   114.30 $ & $    24.00 $ & $  -18.0 $ & $   12.0 $ & $   0.562 $ & FEROS \\
$ 118.62415 $ & $   -42.70 $ & $    28.00 $ & $    3.0 $ & $   13.0 $ & $   0.172 $ & FEROS \\
$ 119.82198 $ & $    39.30 $ & $    37.00 $ & $  -26.0 $ & $   17.0 $ & $   0.565 $ & FEROS \\
$ 126.87056 $ & $   104.30 $ & $    30.00 $ & $   27.0 $ & $   14.0 $ & $   0.881 $ & FEROS \\
$ 144.82638 $ & $   125.30 $ & $    50.00 $ & $  -21.0 $ & $   22.0 $ & $   0.779 $ & FEROS \\
$ 145.89316 $ & $   -98.70 $ & $    45.00 $ & $   91.0 $ & $   20.0 $ & $   0.130 $ & FEROS \\
$ 146.66661 $ & $    14.30 $ & $    47.00 $ & $   35.0 $ & $   21.0 $ & $   0.384 $ & FEROS \\
$ 161.61887 $ & $   -71.98 $ & $    41.00 $ & $  -17.0 $ & $   29.0 $ & $   0.296 $ & Coralie \\
$ 161.70929 $ & $  -121.70 $ & $    32.00 $ & $    9.0 $ & $   15.0 $ & $   0.326 $ & FEROS \\
$ 164.51993 $ & $   -52.98 $ & $    47.00 $ & $  -44.0 $ & $   29.0 $ & $   0.249 $ & Coralie \\
$ 165.67277 $ & $    82.30 $ & $    24.00 $ & $   23.0 $ & $   12.0 $ & $   0.628 $ & FEROS \\
$ 171.58342 $ & $    54.30 $ & $    23.00 $ & $  -10.0 $ & $   12.0 $ & $   0.569 $ & FEROS \\
$ 189.95720 $ & \nodata      & \nodata      & $  -22.0 $ & $   15.8 $ & $   0.605 $ & HDS \\
$ 189.97192 $ & \nodata      & \nodata      & $   -0.3 $ & $   15.3 $ & $   0.610 $ & HDS \\
$ 190.93418 $ & $    43.16 $ & $    15.52 $ & $  -33.5 $ & $   28.3 $ & $   0.928 $ & HDS \\
$ 190.94892 $ & $    43.99 $ & $    12.45 $ & $  -31.0 $ & $   28.4 $ & $   0.932 $ & HDS \\
$ 190.96364 $ & $    12.14 $ & $    18.41 $ & $   13.7 $ & $   21.4 $ & $   0.937 $ & HDS \\
$ 191.93411 $ & $   -66.61 $ & $    25.00 $ & $   11.8 $ & $   21.8 $ & $   0.256 $ & HDS \\
$ 191.94884 $ & $   -40.51 $ & $    25.97 $ & $   28.6 $ & $   19.4 $ & $   0.261 $ & HDS \\
$ 191.96356 $ & $   -75.01 $ & $    31.07 $ & $   16.9 $ & $   41.5 $ & $   0.266 $ & HDS \\
$ 192.92689 $ & $    17.12 $ & $    17.65 $ & $  -18.4 $ & $   18.0 $ & $   0.582 $ & HDS \\
$ 192.93930 $ & $    19.11 $ & $    16.36 $ & $   10.1 $ & $   15.4 $ & $   0.586 $ & HDS \\
$ 192.95172 $ & $    52.12 $ & $    17.50 $ & $   24.2 $ & $   22.9 $ & $   0.590 $ & HDS \\
$ 192.96412 $ & $    48.76 $ & $    23.21 $ & \nodata      & \nodata      & $   0.593 $ & HDS \\
$ 208.70072 $ & $   109.30 $ & $    37.00 $ & $   -8.0 $ & $   17.0 $ & $   0.763 $ & FEROS \\
$ 209.62306 $ & $   -77.70 $ & $    37.00 $ & $  -69.0 $ & $   17.0 $ & $   0.066 $ & FEROS \\
$ 215.61886 $ & $   -28.70 $ & $    33.00 $ & $   78.0 $ & $   15.0 $ & $   0.035 $ & FEROS \\
$ 239.57386 $ & $   137.02 $ & $    43.00 $ & $   63.0 $ & $   26.0 $ & $   0.905 $ & Coralie \\
$ 240.56437 $ & \nodata      & \nodata      & $ -120.0 $ & $   37.0 $ & $   0.230 $ & Coralie \\


==> newcommand_gen.tex <==
%%GB: General commands to make editing easier and with less typos.

%% -----------------------------------------------
%% Definition of a forloop command
%%
%% This is called via: 
%%   \forloop[step]{counter}{initial_value}{conditional}{code_block} 
%%
\newcommand{\forloop}[5][1]%
{%
\setcounter{#2}{#3}%
\ifthenelse{#4}%
	{%
	#5%
	\addtocounter{#2}{#1}%
	\forloop[#1]{#2}{\value{#2}}{#4}{#5}%
	}%
% Else 
	{%
	}%
}% 

%% -----------------------------------------------
%% Editing
\newcommand{\tbd}[1]{{\par\bf\textsc{TBD: #1\\}}}
\newcommand{\ctbd}[1]{}
\newcommand{\cor}{\textcolor{red}{(corr?) }}
\newcommand{\spl}{\textcolor{red}{(spl?) }}

%% ------------------------------------------------
%% Hun characters
\newcommand{\ii}{\'\i }
\newcommand{\oo}{\H{o}}
\newcommand{\uu}{\H u}

%% --------------------------------------
%% Often used. 
\newcommand{\lc}{light curve}
\newcommand{\lcs}{light curves}
\newcommand{\Lc}{Light curve}
\newcommand{\Lcs}{Light curves}
\newcommand{\avg}[1]{\ensuremath{\langle #1\rangle}}
\newcommand{\med}[1]{\ensuremath{\langle #1\rangle_{med}}}
\newcommand{\dpt}{data-point}
\newcommand{\dpts}{data-points}
\newcommand{\tel}{telescope}
\newcommand{\magn}{magnitude}
\newcommand{\stan}{standard}
\newcommand{\aper}{aperture}
\newcommand{\oot}{out-of-transit}
\newcommand{\OOT}{Out-of-Transit}
\newcommand{\cfa}{Harvard-Smithsonian Center for Astrophysics (CfA)}
\newcommand{\cfadigi}{CfA Speedometers}
\newcommand{\cmd}{color-magnitude diagram}

%% ---------------------------------------------
%% 
\newcommand{\conc}[1]{\noindent\par{\noindent{$\mathbf \Longrightarrow$ \bf #1}}}
\newcommand{\diam}{\ensuremath{\oslash}}
\newcommand{\ccdsize}[1]{\ensuremath{\rm #1\times\rm#1}}
\newcommand{\fovsize}[2]{\ensuremath{\rm #1 #2\times\rm#1 #2}}
\newcommand{\tsize}[1]{\mbox{\rm #1 m}}
\newcommand{\band}[1]{\ensuremath{#1}~band}
\newcommand{\ordo}{\ensuremath{\mathcal{O}}}
\newcommand{\chisq}{\ensuremath{\chi^2}}
\newcommand{\RA}[3]{\ensuremath{#1^{\mathrm h}#2^{\mathrm m}#3^{\mathrm s}}}
\newcommand{\DEC}[3]{\ensuremath{#1^{\mathrm d}#2^{\mathrm m}#3^{\mathrm s}}}

%% ---------------------------------------------------------------------
%% Dimensions/quantities
\newcommand{\ghr}{\ensuremath{^h}}
\newcommand{\gmin}{\ensuremath{^m}}
\newcommand{\Ks}{\ensuremath{K_s}}
\newcommand{\masy}{\ensuremath{\rm mas\,yr^{-1}}}
\newcommand{\kms}{\ensuremath{\rm km\,s^{-1}}}
\newcommand{\ms}{\ensuremath{\rm m\,s^{-1}}}
\newcommand{\msd}{\ensuremath{\rm m\,s^{-1}\,d^{-1}}}
\newcommand{\mss}{\ensuremath{\rm m\,s^{-2}}}
\newcommand{\gcmc}{\ensuremath{\rm g\,cm^{-3}}}
\newcommand{\ergscmsq}{\ensuremath{\rm erg\,s^{-1}\,cm^{-2}}}
\newcommand{\C}{\ensuremath{^{\circ}C\;}}
\newcommand{\el}{\ensuremath{e^-}}
\newcommand{\sqarcsec}{\ensuremath{\Box^{\prime\prime}}}
\newcommand{\sqarcdeg}{\ensuremath{\Box^{\circ}}}
\newcommand{\pxs}{\ensuremath{\rm \arcsec pixel^{-1}}}
\newcommand{\aduel}{\ensuremath{\lbrack ADU/\el \rbrack}}
\newcommand{\eladu}{\ensuremath{\lbrack \el/ADU \rbrack}}
\newcommand{\adupixs}{\ensuremath{\rm ADU/(pix\, s)}}
\newcommand{\elpixs}{\ensuremath{\rm \el/(pix\, s)}}
\newcommand{\masyr}{\ensuremath{\rm mas\,yr^{-1}}}

%% ---------------------------------------------------------------------
%% General
\newcommand{\msini}{\ensuremath{m \sin i}}
\newcommand{\mplsini}{\ensuremath{\mpl\sin i}}
\newcommand{\teff}{\ensuremath{T_{\rm eff}}}
\newcommand{\logg}{\ensuremath{\log{g}}}
\newcommand{\vsini}{\ensuremath{v \sin{i}}}
\newcommand{\feh}{\ensuremath{\rm [Fe/H]}}
\newcommand{\logl}{\ensuremath{\log{L}}}
\newcommand{\vmac}{\ensuremath{v_{\rm mac}}}
\newcommand{\vmic}{\ensuremath{v_{\rm mic}}}
% Activity index R'_HK
\newcommand{\rhk}{\ensuremath{R^{\prime}_{\rm HK}}}
% log of R'_HK
\newcommand{\logrhk}{\ensuremath{\log\rhk}}
% S average value
\newcommand{\Savg}{\ensuremath{\langle S\rangle}}
% Some magnitude differences
\newcommand{\vic}{\ensuremath{V\!-\!I_C}}
\newcommand{\ebv}{\ensuremath{E(B\!-\!V)}}

%% ---------------------------------------------------------------------
%% Solar quantities 
\newcommand{\rsun}{\ensuremath{R_\sun}}
\newcommand{\msun}{\ensuremath{M_\sun}}
\newcommand{\lsun}{\ensuremath{L_\sun}}
\newcommand{\loglsun}{\ensuremath{\log{L_\sun}}}
\newcommand{\teffsun}{\ensuremath{T_{eff,\sun}}}
\newcommand{\rhosun}{\ensuremath{\rho_\sun}}
\newcommand{\loggsun}{\ensuremath{\log{g_{\sun}}}}

%% ---------------------------------------------------------------------
%% Stellar quantities 
\newcommand{\rstar}{\ensuremath{R_\star}}
\newcommand{\mstar}{\ensuremath{M_\star}}
\newcommand{\lstar}{\ensuremath{L_\star}}
\newcommand{\astar}{\ensuremath{a_\star}}
\newcommand{\loglstar}{\ensuremath{\log{L_\star}}}
\newcommand{\teffstar}{\ensuremath{T_{\rm eff\star}}}
\newcommand{\rhostar}{\ensuremath{\rho_\star}}
\newcommand{\loggstar}{\ensuremath{\log{g_{\star}}}}

%% ---------------------------------------------------------------------
%% Earth
\newcommand{\rearth}{\ensuremath{R_\earth}}
\newcommand{\mearth}{\ensuremath{M_\earth}}
\newcommand{\learth}{\ensuremath{L_\earth}}
\newcommand{\teffearth}{\ensuremath{T_{\rm eff,\earth}}}
\newcommand{\rhoearth}{\ensuremath{\rho_\earth}}

%% ---------------------------------------------------------------------
%% Planetary
\newcommand{\rpl}{\ensuremath{R_{p}}}
\newcommand{\mpl}{\ensuremath{M_{p}}}
\newcommand{\lpl}{\ensuremath{L_{p}}}
\newcommand{\teffpl}{\ensuremath{T_{\rm eff,{p}}}}
\newcommand{\rhopl}{\ensuremath{\rho_{p}}}
\newcommand{\ipl}{\ensuremath{i_{p}}}
\newcommand{\epl}{\ensuremath{e_{p}}}
\newcommand{\gpl}{\ensuremath{g_{p}}}
\newcommand{\loggpl}{\ensuremath{\log g_{p}}}

\newcommand{\arstar}{\ensuremath{a/\rstar}}
\newcommand{\zrstar}{\ensuremath{\zeta/\rstar}}

%% ---------------------------------------------------------------------
%% Jupiter
\newcommand{\rjup}{\ensuremath{R_{\rm J}}}
\newcommand{\mjup}{\ensuremath{M_{\rm J}}}
\newcommand{\ljup}{\ensuremath{L_{\rm J}}}
\newcommand{\teffjup}{\ensuremath{T_{eff,{\rm J}}}}
\newcommand{\rhojup}{\ensuremath{\rho_{\rm J}}}
\newcommand{\gjup}{\ensuremath{\g_{\rm J}}}

\newcommand{\rjuplong}{\ensuremath{R_{\rm Jup}}}
\newcommand{\mjuplong}{\ensuremath{M_{\rm Jup}}}
\newcommand{\ljuplong}{\ensuremath{L_{\rm Jup}}}
\newcommand{\teffjuplong}{\ensuremath{T_{eff,{\rm Jup}}}}
\newcommand{\rhojuplong}{\ensuremath{\rho_{\rm Jup}}}
\newcommand{\gjuplong}{\ensuremath{\g_{\rm Jup}}}

%% -----------------------------
%% Software
\newcommand{\pack}[1]{\textsc{\lowercase{#1}}}
\newcommand{\prog}[1]{\texttt{\lowercase{#1}}}
\newcommand{\iraf}{\pack{iraf}}
\newcommand{\todcor}{\prog{todcor}}
\newcommand{\xcsao}{\prog{xcsao}}
\newcommand{\daophot}{\pack{daophot}}
\newcommand{\fihat}{\pack{fihat}}
\newcommand{\fistar}{\prog{fistar}}
\newcommand{\fiphot}{\prog{fiphot}}
\newcommand{\grmatch}{\prog{grmatch}}
\newcommand{\grtrans}{\prog{grtrans}}

%% ---------------------------------------
%% References
%\newcommand{\pref}[1]{p.~\pageref{#1}}
%\newcommand{\figr}[1]{Fig.~\ref{fig:#1}}
%\newcommand{\secr}[1]{\mbox{\S\ \ref{sec:#1}}}
%\newcommand{\eqr}[1]{Eq.~\ref{eq:#1}}
%\newcommand{\tabsr}[1]{Tab.~\ref{tab:#1}}
%\newcommand{\tabr}[1]{\mbox{Table~\ref{tab:#1}}}
%\newcommand{\figrp}[1]{Fig.~\ref{fig:#1} on \pref{fig:#1}}
%\newcommand{\secrp}[1]{\S\ref{sec:#1} on \pref{sec:#1}}
%\newcommand{\eqrp}[1]{Eq.~\ref{eq:#1} on \pref{eq:#1}}
%\newcommand{\tabrp}[1]{Tab.~\ref{tab:#1} on \pref{tab:#1}}

\newcommand{\refp}[1]{p.~\pageref{#1}}

\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\refsec}[1]{\mbox{\S\ \ref{sec:#1}}}
\newcommand{\refeq}[1]{Eq.~\ref{eq:#1}}
\newcommand{\reftab}[1]{Tab.~\ref{tab:#1}}

\newcommand{\reffigl}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsecl}[1]{\mbox{Section \ref{sec:#1}}}
\newcommand{\refeql}[1]{Equation~\ref{eq:#1}}
\newcommand{\reftabl}[1]{Table~\ref{tab:#1}}

\newcommand{\reffigp}[1]{\reffig{#1} on \pref{fig:#1}}
\newcommand{\refsecp}[1]{\refsec{#1} on \pref{sec:#1}}
\newcommand{\refeqp}[1]{\refeq{#1} on \pref{eq:#1}}
\newcommand{\reftabp}[1]{\reftab{#1} on \pref{tab:#1}}

\newcommand{\reffigls}[2]{Figures~\ref{fig:#1}-\ref{fig:#2}}
\newcommand{\reftabls}[2]{Tables~\ref{tab:#1}-\ref{tab:#2}}

%% --------------------------------------
%% Instruments
% 
%% FLWO 1.2 m telescope
\newcommand{\flwof}{\mbox{FLWO 1.2\,m}}

%% FLWO 1.5 m telescope
\newcommand{\flwos}{\mbox{FLWO 1.5\,m}}

%% TopHAT 0.25m telescope
\newcommand{\flwot}{\mbox{TopHAT 0.25\,m}}

%% MMT
\newcommand{\mmt}{\mbox{MMT 6.5\,m}}

%% Spitzer
\newcommand{\ssts}{{\em Spitzer}}
\newcommand{\sstL}{{\em Spitzer Space Telescope}}

%% HST
\newcommand{\hst}{{\em HST}}

%% Wise 1m
\newcommand{\wom}{\mbox{Wise 1\,m}}

\newcommand{\piszkessch}{Konkoly 0.6\,m Schmidt}
\newcommand{\piszkesrcc}{Konkoly 1\,m RCC}


%% --------------------------------------
%% Variable types
%% 
\newcommand{\dscu}{\mbox{$\delta$ Scuti}}
\newcommand{\gdor}{\mbox{$\gamma$ Dor}}

\newcommand{\hj}{hot Jupiter}
\newcommand{\vhj}{very hot Jupiter}

% ---------------------------------------------------------------------
%% Astronomical catalogues

%% HD: 
\newcommand{\hd}[1]{\mbox{HD #1}}

%% BD
\newcommand{\BD}[1]{\mbox{BD #1}}

%% HIP
\newcommand{\hip}[1]{\mbox{HIP #1}}

%% GJ
\newcommand{\gj}[1]{\mbox{GJ #1}}

% ---------------------------------------------------------------------
% Shorthand
\newcommand{\tbn}[1]{\tablenotemark{#1}}


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxx below with a unique identifier for each planet (e.g. xxxxA for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxA. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxx}{HAT-P-14}
\newcommand{\hatcurbxxxxx}{HAT-P-14b}
\newcommand{\hatcurcxxxxx}{HAT-P-14c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxx}{14}

%\newcommand{\hatcurCCraxxxxx}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxx}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxx}{\hatcurDSgamma{\hatcurplanetnumxxxxx}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxx}{\hatcurRVgamma{\hatcurplanetnumxxxxx}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxx}{\ensuremath{0.527\pm0.12}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxx}{ii}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxx}{YY}
%\newcommand{\hatcurisoshortxxxxx}{Baraffe}
\newcommand{\hatcurisofullxxxxx}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxx}{Baraffe}
\newcommand{\hatcurisocitexxxxx}{yi:2001}
%\newcommand{\hatcurisocitexxxxx}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxx}{\arstar}
%\newcommand{\hatcurlumindxxxxx}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxx}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxx}{BB}
%\newcommand{\hatcurjhkfilsetxxxxx}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxxx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxx}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehshortxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEloggxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxx}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvsinxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxx}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmacxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmicxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxx}}}

